Faster Randomized Interior Point Methods for Tall/Wide Linear Programs

Linear programming (LP) is an extremely useful tool which has been successfully applied to solve various problems in a wide range of areas, including operations research, engineering, economics, or even more abstract mathematical areas such as combinatorics. It is also used in many machine learning applications, such as $\ell_1$-regularized SVMs, basis pursuit, nonnegative matrix factorization, etc. Interior Point Methods (IPMs) are one of the most popular methods to solve LPs both in theory and in practice. Their underlying complexity is dominated by the cost of solving a system of linear equations at each iteration. In this paper, we consider both feasible and infeasible IPMs for the special case where the number of variables is much larger than the number of constraints. Using tools from Randomized Linear Algebra, we present a preconditioning technique that, when combined with the iterative solvers such as Conjugate Gradient or Chebyshev Iteration, provably guarantees that IPM algorithms (suitably modified to account for the error incurred by the approximate solver), converge to a feasible, approximately optimal solution, without increasing their iteration complexity. Our empirical evaluations verify our theoretical results on both real-world and synthetic data.

==> Definitions.tex <==
% 2014 written by S V N Vishwanathan (vishy@ucsc.edu)
% 2015 modified by Jiasen Yang (jiaseny@purdue.edu)

\RequirePackage{latexsym}
\RequirePackage{amsmath}
% \RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage[mathscr]{euscript}

\newcommand{\D}{\text{d}}
\newcommand{\ex}{\mathbb{E}}
\newcommand{\Ex}[1]{\mbox{}\mathbb{E}\left[#1\right]}
\newcommand{\Var}[1]{\mbox{}\textup{Var}\left(#1\right)}
\newcommand{\Cov}[1]{\mbox{}\textup{Cov}\left(#1\right)}
\newcommand{\Tr}[1]{\mbox{}\textup{tr}\left(#1\right)}
\newcommand{\Trsq}[1]{\mbox{}\textup{tr}^2\left(#1\right)}
% \newcommand{\pr}{\mathbb{P}}
\newcommand{\pr}[1]{\mbox{}\mathbb{P}\left(#1\right)}
\newcommand{\kl}[2]{\mbox{}\mathbb{KL}\left(#1\,||\,#2\right)}
\newcommand{\tAb}{\widetilde{\Ab}}
\newcommand{\tp}{\widetilde{p}}
\newcommand{\ts}{\mathsf{T}}
% \newcommand{\ts}{\top}
% \newcommand{\ind}[1]{\mathbb{I}\{#1\}}
\newcommand{\ind}[1]{\mathds{1}\{#1\}}
\newcommand{\nnz}[1]{\mathsf{nnz}(#1)}
\newcommand{\Diag}[1]{\diag \left\{#1\right\}} % pseudoinverse
\newcommand{\Pinv}[1]{\mbox{}\left(#1\right)^{\dagger}} % pseudoinverse
\newcommand{\inv}[1]{\mbox{}\left(#1\right)^{-1}} % pseudoinverse
\newcommand{\RR}[2]{\mathbb{R}^{#1 \times #2}} % Real numbers
\newcommand{\R}[1]{\mathbb{R}^{#1}} % Real numbers
\newcommand{\Sqrt}[1]{#1^{\nicefrac{1}{2}}} % pseudoinverse
\newcommand{\defeq}{\triangleq}
% \newcommand{\var}{\text{var}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\disteq}{\stackrel{d}{=}}
\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\todo}[1]{\textcolor{red}{\texttt{TODO}: \emph{#1}}}


%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cbb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

% \newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Abtil}{\widetilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Ascr}{\mathscr{A}}
\newcommand{\Bscr}{\mathscr{B}}
\newcommand{\Cscr}{\mathscr{C}}
\newcommand{\Dscr}{\mathscr{D}}
\newcommand{\Escr}{\mathscr{E}}
\newcommand{\Fscr}{\mathscr{F}}
\newcommand{\Gscr}{\mathscr{G}}
\newcommand{\Hscr}{\mathscr{H}}
\newcommand{\Iscr}{\mathscr{I}}
\newcommand{\Jscr}{\mathscr{J}}
\newcommand{\Kscr}{\mathscr{K}}
\newcommand{\Lscr}{\mathscr{L}}
\newcommand{\Mscr}{\mathscr{M}}
\newcommand{\Nscr}{\mathscr{N}}
\newcommand{\Oscr}{\mathscr{O}}
\newcommand{\Pscr}{\mathscr{P}}
\newcommand{\Qscr}{\mathscr{Q}}
\newcommand{\Rscr}{\mathscr{R}}
\newcommand{\Sscr}{\mathscr{S}}
\newcommand{\Tscr}{\mathscr{T}}
\newcommand{\Uscr}{\mathscr{U}}
\newcommand{\Vscr}{\mathscr{V}}
\newcommand{\Wscr}{\mathscr{W}}
\newcommand{\Xscr}{\mathscr{X}}
\newcommand{\Yscr}{\mathscr{Y}}
\newcommand{\Zscr}{\mathscr{Z}}

\newcommand{\Ascrb}{\boldsymbol{\Ascr}}
\newcommand{\Bscrb}{\boldsymbol{\Bscr}}
\newcommand{\Cscrb}{\boldsymbol{\Cscr}}
\newcommand{\Dscrb}{\boldsymbol{\Dscr}}
\newcommand{\Escrb}{\boldsymbol{\Escr}}
\newcommand{\Fscrb}{\boldsymbol{\Fscr}}
\newcommand{\Gscrb}{\boldsymbol{\Gscr}}
\newcommand{\Hscrb}{\boldsymbol{\Hscr}}
\newcommand{\Iscrb}{\boldsymbol{\Iscr}}
\newcommand{\Jscrb}{\boldsymbol{\Jscr}}
\newcommand{\Kscrb}{\boldsymbol{\Kscr}}
\newcommand{\Lscrb}{\boldsymbol{\Lscr}}
\newcommand{\Mscrb}{\boldsymbol{\Mscr}}
\newcommand{\Nscrb}{\boldsymbol{\Nscr}}
\newcommand{\Oscrb}{\boldsymbol{\Oscr}}
\newcommand{\Pscrb}{\boldsymbol{\Pscr}}
\newcommand{\Qscrb}{\boldsymbol{\Qscr}}
\newcommand{\Rscrb}{\boldsymbol{\Rscr}}
\newcommand{\Sscrb}{\boldsymbol{\Sscr}}
\newcommand{\Tscrb}{\boldsymbol{\Tscr}}
\newcommand{\Uscrb}{\boldsymbol{\Uscr}}
\newcommand{\Vscrb}{\boldsymbol{\Vscr}}
\newcommand{\Wscrb}{\boldsymbol{\Wscr}}
\newcommand{\Xscrb}{\boldsymbol{\Xscr}}
\newcommand{\Xscrbh}{\hat{\Xscrb}}
\newcommand{\Yscrb}{\boldsymbol{\Yscr}}
\newcommand{\Zscrb}{\boldsymbol{\Zscr}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}
\newcommand{\Lmat}{\Lb}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}

\newcommand{\vol}{\text{vol}}
\newcommand{\Ocaltil}{\widetilde{\mathcal{O}}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}[theorem]{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}[theorem]{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
% \newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
% \newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{iid}}
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\cf}{\emph{cf.}\ }

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
% \newcommand{\ind}{\boldsymbol{\mathsf{I}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}
\newcommand{\Thetab}{\mathbf{\Theta}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}
\newcommand{\Lambdab}{\mathbf{\Lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}
\newcommand{\Omegab}{\boldsymbol{\Omega}}
\newcommand{\Phib}{\boldsymbol{\Phi}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ve}{\varepsilon}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


\newcommand{\Aone}{\textbf{A1}}
\newcommand{\Atwo}{\textbf{A2}}

\newcommand{\hWb}{\widehat{\Wb}}
% \newcommand{\Sreg}{\Sigmab_\mathsf{reg}}
\newcommand{\Sreg}{\widetilde{\Sigmab}}



%-----------------------------
% Palma's commands 
\newcommand{\agniva}[1]{\textcolor{ForestGreen}{[Agniva: #1]}}
\newcommand{\palma}[1]{\textcolor{blue}{[Palma: #1]}}
\newcommand{\haim}[1]{\textcolor{red}{[Haim: #1]}}
\newcommand{\bl}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\brown}[1]{\textcolor{brown}{#1}}

\newcommand{\dimone}{m}
\newcommand{\dimtwo}{n}

\newcommand{\sig}{\sigma}
\newcommand{\sigmin}{\underline{\sigma}}
\newcommand{\sigmax}{\overline{\sigma}}

%\newcommand{\alphatil}{\tilde{\alpha}} // already above
\newcommand{\alphabar}{\bar{\alpha}}

\newcommand{\neigh}{\mathcal{N}(\gamma)}


\newcommand{\Delx}{\Delta \xb}
\newcommand{\Dels}{\Delta \sbb}
\newcommand{\Dely}{\Delta \yb}

\newcommand{\xnew}{\xb(\alpha)}
\newcommand{\snew}{\sbb(\alpha)}
\newcommand{\ynew}{\yb(\alpha)}
\newcommand{\munew}{\mu(\alpha)}
\newcommand{\rnew}{r(\alpha)}

\newcommand{\delxdels}{\hat{\Delta \xb} \circ \hat{\Delta \sbb} }
\newcommand{\delxTdels}{\hat{\Delta\xb}^\ts \hat{\Delta \sbb} }
\newcommand{\xcircs}{\xb \circ \sbb }
\newcommand{\delxdelsnorm}{\|\hat{\Delta \xb} \circ \hat{\Delta \sbb} \|_\infty}

\newcommand{\threefac}{\gamma \sig \mu}
\newcommand{\vTen}{\vb^\ts \one_\dimtwo / \dimtwo}
\newcommand{\vTenfrac}{\frac{\vb^\ts \one_\dimtwo}{\dimtwo}}

\newcommand{\alphamax}{\tilde{\alpha}}
\newcommand{\alphaused}{\bar{\alpha}}

\newcommand{\fapprox}{\tilde{f}}

\newcommand{\factorone}{B}
\newcommand{\factortwo}{A}


%----------------------------
% Experiments 
\newcommand{\tolCG}[0]{$\emph{tolCG}$} % 
\newcommand{\tolOuterRes}[0]{$\tau$}

\newcommand{\precNormal}[0]{$\Qb^{-\nicefrac{1}{2}}\Ab\Db^2\Ab^\ts\Qb^{-\nicefrac{1}{2}}$}

\newcommand{\kprecNormal}[0]{$\kappa(\Qb^{-\nicefrac{1}{2}}\Ab\Db^2\Ab^\ts\Qb^{-\nicefrac{1}{2}}$)}


==> X_feasible.tex <==
\section{Feasible IPM}
\subsection{The linear system}
Let $\mathcal{F}$ and $\mathcal{F}^0$ be the sets of feasible and strictly feasible points respectively \ie,
\begin{flalign*}
\mathcal{F}=&~\{(\xb,\yb,\sbb):~(\xb,\sbb)\ge\zero,~\Ab\xb=\bb,~\Ab^\ts\yb+\sbb=\cbb\}\nonumber\\
\mathcal{F}^0=&~\{(\xb,\yb,\sbb): ~(\xb,\sbb)>\zero,~\Ab\xb=\bb,~\Ab^\ts\yb+\sbb=\cbb\}.
\end{flalign*}
In addition, let the neighborhood $\mathcal{N}(\gamma)$ be
%
\begin{flalign}
&\mathcal{N}(\gamma)=\Big\{(\xb,\yb,\sbb)\in\mathcal{F}^0:x_i s_i\ge(1-\gamma)\mu\Big\}.\nonumber
\end{flalign}
%
Here $\gamma \in (0,1)$ and $\mu$ is the duality measure.
Note that $\mathcal{N}(\gamma)\subseteq\mathcal{F}^0\subseteq\mathcal{F}$. We assume that $\mathcal{F}^0$ is non-empty.
%
At each iteration, given the current solution $(\xb^{k},\yb^{k},\sbb^{k})$, IPMs obtain the search direction $(\Delta\xb^k,\Delta\yb^k,\Delta\sbb^k)$ by solving the following system of linear equations:
\begin{subequations}\label{eq:system_f}
	\begin{flalign}
	\Ab\Db^2\Ab^\ts\Delta\yb=~&\pb\,,\label{eq:normal1_f}\\
	\Delta\sbb=~&-\Ab^\ts\Delta\yb^k\,,\label{eq:dels_f}\\
	\Delta\xb=~&-\xb+\sigma\mu\Sb^{-1}\one_\dimtwo-\Db^2\Delta\sbb\,,\label{eq:delx_f}
	\end{flalign}
\end{subequations}
%
where $\pb=-\sigma\mu\Ab\Sb^{-1}\one_\dimtwo+\Ab\xb$.
%
%\begin{flalign}\label{eqn:pdef}
%
%\pb^k&=-\rb_p^k-\sigma\mu_k\Ab\Sb^{-1}\one_\dimtwo+\Ab\xb^k-\Ab\Db^2\rb^k_d.
%
%\end{flalign}
%
%
Given $\Delta\yb$ from eqn.~(\ref{eq:normal1_f}), $\Delta\sbb$ and $\Delta\xb$ are easy to compute from eqns.~\eqref{eq:dels_f} and \eqref{eq:delx_f}, as they only involve matrix-vector products.  Note that we solve eqn.~\eqref{eq:normal1_f} approximately using a sketching-based preconditioned CG solver. Let $\hat{\Delta \yb}=\Qb^{\nicefrac{-1}{2}}\tilde{\zb}^t$ be the approximate solution to eqn.~(\ref{eq:normal1_f}). In order to account for the loss of accuracy due to this approximate solution, we compute $\hat{\Delta\xb}$ as follows:
%
\begin{flalign}
\hat{\Delta\xb}=~-\xb+\sigma\mu\Sb^{-1}\one_\dimtwo-\Db^2\hat{\Delta\sbb}-\Sb^{-1}\vb\label{eq:delxhat_f}.
\end{flalign}
%
Here $\vb\in\R{n}$ is a perturbation vector that needs to exactly satisfy the following invariant at each iteration of the IPM:
%
\begin{flalign}
%
\Ab\Sb^{-1}\vb=\Ab\Db^2\Ab^\ts\hat{\Delta\yb}-\pb\,\label{eq:addl_f}.
%
\end{flalign}
%
We note that the computation of $\hat{ \Delta \sbb}$ is still done using eqn.~\eqref{eq:dels_f}, which does not change. Therefore, we rewrite the approximate solution $(\hat{\Delta\xb},\hat{\Delta\yb},\hat{\Delta\sbb})$ together with the perturbation vector $\vb\in\R{n}$ satisfying eqn.~\eqref{eq:addl_f} as follows:
%
\begin{subequations}\label{eq:system1}
	\begin{flalign}
	\Ab\Db^2\Ab^\ts\hat{\Delta\yb}=~&\pb+\Ab\Sb^{-1}\vb\,,\label{eq:normal12}\\
	\hat{\Delta\sbb}=~&-\Ab^\ts\hat{\Delta\yb}\,,\label{eq:dels1}\\
	\hat{\Delta\xb}=~&-\xb+\sigma\mu\Sb^{-1}\one_\dimtwo-\Db^2\hat{\Delta\sbb}-\Sb^{-1}\vb\label{eq:delxhat1}\,.
	\end{flalign}
\end{subequations}

\noindent\textbf{Bounding the norm of $\vb$.} We note that using the same analysis as in the case of infeasible IPMs, it can be shown that we need $t=\Ocal(\log n)$ iterations to guarantee $$\|\vb\|_2\le\frac{\gamma\sigma\mu}{4}.$$

\subsection{Structural conditions}
Recall that our preconditioner $\Qb^{-\frac{1}{2}}$ satisfies
%
\begin{flalign}\label{eq:pdcond1_f}
\frac{2}{2+\zeta} \leq \sigma^2_{\min}(\Qb^{-\frac{1}{2}}\Ab\Db) \leq \sigma^2_{\max}(\Qb^{-\frac{1}{2}}\Ab\Db) \leq \frac{2}{2-\zeta},
\end{flalign}
%
for some error parameter $\zeta \in  [0,1]$. In the above, $\sigma_{\min}(\cdot)$ and $\sigma_{\max}(\cdot)$ correspond to the smallest and largest singular value of the matrix in parentheses. Moreover, given such a preconditioner, we prove that the resulting iterative solver satisfies
%
\begin{flalign}
\|\tilde{\fb}^{(t)}\|_2=\|\Qb^{-\nicefrac{1}{2}}\Ab\Db^2\Ab^\ts\Qb^{-\nicefrac{1}{2}}\tilde{\zb}^t-\Qb^{-\nicefrac{1}{2}}\pb\|_2\leq
\zeta^t \|\Qb^{-\nicefrac{1}{2}}\pb\|_2. \label{eq:pdcond2_f}
\end{flalign}
%
Here $\tilde{\zb}^t$ is the approximate solution returned by the iterative solver after $t$ iterations.

% \subsection{Bounding \texorpdfstring{$\|\Qb^{-\nicefrac{1}{2}}\pb\|_2$}{Lg} and number of inner iterations}
% \begin{lemma}\label{thm:boundf_f}
% 	Let $(\xb,\yb,\sbb)\in\mathcal{N}(\gamma)$ and let the sketching matrix $\Wb\in\RR{\dimtwo}{w}$ satisfy the condition in eqn.~\eqref{eq:pdcond1}. Then,
% 	\begin{flalign}
% 	\|\Qb^{-\nicefrac{1}{2}}\pb\|_2\le~\left(1+ \frac{\sigma}{\sqrt{1-\gamma}}\right)\sqrt{2n\mu}\,.
% 	\end{flalign}
% \end{lemma}

% \begin{proof}	
% 	To bound $\|\Qb^{-\nicefrac{1}{2}}\pb\|_2$,  first we express $\pb$ as in eqn.~\eqref{eq:system_f} and rewrite
% 	\begin{flalign}
% 	\Qb^{-\nicefrac{1}{2}}\pb
% 	=&~\Qb^{-\nicefrac{1}{2}}\left(-\sigma\mu\Ab\Sb^{-1}\one_\dimtwo+\Ab\xb\right)\label{eq:recur3_f}.
% 	\end{flalign}
% %	
% Applying the triangle inequality on $\|\Qb^{-\nicefrac{1}{2}}\pb\|_2$ in eqn.~\eqref{eq:recur3_f}, we get
% 	\begin{flalign}
% 	\|\Qb^{-\nicefrac{1}{2}}\pb\|_2\le \Delta_1+\Delta_2\label{eq:recur4_f}\,,
% 	\end{flalign}
% 	where $\Delta_1=~\sigma\mu\|\Qb^{-\nicefrac{1}{2}}\Ab\Db(\Xb\Sb)^{-\nicefrac{1}{2}}\one_\dimtwo\|_2$ and
% 	$\Delta_2=~\|\Qb^{-\nicefrac{1}{2}}\Ab\Db\Db^{-1}\xb\|_2$.
% %
% 	In order to bound  $\Delta_1$ and $\Delta_2$, we use the condition of eqn.~\eqref{eq:pdcond1_f}. In particular, eqn.~\eqref{eq:pdcond1_f} implies that $\|\Qb^{-\nicefrac{1}{2}}\Ab\Db\|_2\le\sqrt{2}$ as $\zeta\le 1$.
	
% 	\paragraph{Bounding $\Delta_1$.} Applying submultiplicativity, we get
% 	\begin{flalign}
% 	\Delta_1=&~\sigma\mu\,\|\Qb^{-\nicefrac{1}{2}}\,\Ab\Db\,(\Xb\Sb)^{-\nicefrac{1}{2}}\one_\dimtwo\|_2\nonumber\\
% 	\le&~\sigma\mu\,\|\Qb^{-\nicefrac{1}{2}}\,\Ab\Db\|_2\|(\Xb\Sb)^{-\nicefrac{1}{2}}\one_\dimtwo\|_2\nonumber\\
% 	\le&~\sqrt{2}\,\sigma\mu\,\|(\Xb\Sb)^{-\nicefrac{1}{2}}\one_\dimtwo\|_2\nonumber\\
% 	=&~\sqrt{2}\,\sigma\mu\,\sqrt{\sum_{i=1}^{\dimtwo}\frac{1}{x_i s_i}}
% 	\le~\sqrt{2}\,\sigma\mu\,\sqrt{\sum_{i=1}^{\dimtwo}\frac{1}{(1-\gamma)\mu}}\nonumber\\
% 	=&~\sqrt{2}\,\sigma\,\sqrt{\frac{\dimtwo\,\mu}{(1-\gamma)}}\label{eq:del2_f}\,,
% 	\end{flalign}
% 	where we used the fact that $(\xb,\yb,\sbb)\in\mathcal{N}(\gamma)$.
	
% 	\paragraph{Bounding $\Delta_2$.} Since $\Db=\Sb^{-\nicefrac{1}{2}}\Xb^{\nicefrac{1}{2}}$ and $\xb=\Xb\,\one_\dimtwo$, we get
% 	%
% 	\begin{flalign}
% 	\Delta_2=&~\|\Qb^{-\nicefrac{1}{2}}\,\Ab\Db\,(\Sb^{\nicefrac{1}{2}}\Xb^{-\nicefrac{1}{2}})\,\Xb\,\one_\dimtwo\|_2\nonumber\\
% 	=&~\|\Qb^{-\nicefrac{1}{2}}\,\Ab\Db\,(\Sb\Xb)^{\nicefrac{1}{2}}\,\one_\dimtwo\|_2\nonumber\\
% 	\le&~\|\Qb^{-\nicefrac{1}{2}}\,\Ab\Db\|_2\|(\Sb\Xb)^{\nicefrac{1}{2}}\,\one_\dimtwo\|_2\nonumber\\
% 	\le&~\sqrt{2}\,\sqrt{\sum_{i=1}^{\dimtwo}x_i s_i}=~\sqrt{2\dimtwo\,\mu}\label{eq:del3_f}.
% 	\end{flalign}

% 	\paragraph{Final bound.} Combining eqns.~\eqref{eq:recur4_f},~\eqref{eq:del2_f}, and~\eqref{eq:del3_f}, we get
% 	\begin{flalign}
% 	\|\Qb^{-\nicefrac{1}{2}}\pb\|_2\le~\left(1+ \frac{\sigma}{\sqrt{1-\gamma}}\right)\sqrt{2n\mu}\,.
% 	\end{flalign}
% 	This concludes the proof of Lemma~\ref{thm:boundf_f}.
% \end{proof}

% \subsection{Convergence analysis}
% %\begin{flalign}
% %
% %$\Ab\Sb^{-1}\vb=\Ab\Db^2\Ab^\ts\hat{\Delta\yb}-\pb\,\label{eq:addl}.$
% %
% %\end{flalign}
% We can rewrite the linear system of eqn.~\eqref{eq:system1} as follows:
% %
% \begin{subequations}\label{eq:iip_3_f}
% 	\begin{flalign}
% 	\Ab\hat{\Delta\xb}=&~\zero, \label{eq:iip_3_f_1}\\
% 	\Ab^\ts\hat{\Delta\yb}+\hat{\Delta\sbb}=&~\zero,  \label{eq:iip_3_f_2}\\
% 	\Xb\hat{\Delta\sbb}+\Sb\hat{\Delta\xb}=&-\Xb\Sb\,\one_\dimtwo+\sigma\mu\,\one_\dimtwo - \vb.  \label{eq:iip_3_f_3}
% 	\end{flalign}
% \end{subequations}
% %
% Indeed, we now show how to derive eqn.~\eqref{eq:system1} from eqn.~\eqref{eq:iip_3_f}. Pre-multiplying both sides of eqn.~\eqref{eq:iip_3_f_3} by $\Ab\Sb^{-1}$ and noting that $\Db^2=\Xb\Sb^{-1}$, we get
% %
% \begin{flalign}
% &~\Ab\Db^2\hat{\Delta\sbb}+\Ab\hat{\Delx}=-\Ab\Xb\one_n+\sigma\mu\Ab\Sb^{-1}\one_n-\Ab\Sb^{-1}\vb\nonumber\\
% \Rightarrow&~\Ab\Db^2\hat{\Delta\sbb}=-\Ab\xb+\sigma\mu\Ab\Sb^{-1}\one_n-\Ab\Sb^{-1}\vb.\label{eq:iip_3_f1}
% \end{flalign}
% %
% Eqn.~\eqref{eq:iip_3_f1} holds as $\Ab\Xb\one_n=\Ab\xb$ and, from eqn.~\eqref{eq:iip_3_f_1}, $\Ab\hat{\Delx}=\zero$. Next, pre-multiplying eqn.~\eqref{eq:iip_3_f_2} by $\Ab\Db^2$, we get
% %
% \begin{flalign}
% &~\Ab\Db^2\Ab^\ts\hat{\Dely}+\Ab\Db^2\hat{\Dels}=\zero\nonumber\\
% \Rightarrow &~\Ab\Db^2\Ab^\ts\hat{\Dely}=\Ab\xb-\sigma\mu\Ab\Sb^{-1}\one_n+\Ab\Sb^{-1}\vb=\pb+\Ab\Sb^{-1}\vb.\label{eq:iip_3_f11}
% \end{flalign}
% %
% The first equality in eqn.~\eqref{eq:iip_3_f11} follows from eqn.~\eqref{eq:iip_3_f1} and the definition of $\pb$. This establishes
% eqn.~\eqref{eq:normal12}. Eqn.~\eqref{eq:dels1} directly follows from eqn.~\eqref{eq:iip_3_f_2}. Finally, we get eqn.~\eqref{eq:delxhat1} by pre-multiplying eqn.~\eqref{eq:iip_3_f_3} by $\Sb^{-1}$.
% %
% We define the next point traversed by the algorithm as $(\xnew,\ynew, \snew)$, where
% \begin{flalign}
% (\xnew,\ynew,\snew) &= (\xb, \yb, \sbb) + \alpha(\hat{\Delta\xb},\hat{\Delta \yb},\hat{\Delta\sbb}),\ \mbox{and} \\
% \munew &= \left(\nicefrac{1}{n}\right)\xnew^\ts \snew.
% \end{flalign}
% %
% Our goal is to bound the number of outer iterations required by the feasible IPM algorithm.
% To do so, we bound the magnitude of the step size $\alpha$. First, we provide an upper bound on $\alpha$, which allows us to show that each new point $(\xnew,\ynew,\snew)$ traversed by the algorithm stays within the neighborhood $\neigh$.
% Second, we provide a lower bound on $\alpha$, which allows us to bound the number of iterations required. 
% %
% The following Lemma will be used throughout the section.
% %
% \begin{lemma}\label{lemmamaxalpha0}
% 	Assume $(\hat{\Delx},\hat{\Dels},\hat{\Dely})$ satisfies eqns. $(\ref{eq:iip_3})$ for some $\sig \in \mathbb{R}$ and $\vb \in \mathbb{R}^\dimtwo$. Let $(\xb,\yb,\sbb)$ be any point such that $(\xb,\sbb)>0$. Then, for every $\alpha \in \mathbb{R}$, 
% 	%
% 	\begin{flalign*}
% 	(a)&~~\xnew \circ \snew = (1- \alpha) \xcircs + \alpha \sig \mu \one_\dimtwo - \alpha \vb + \alpha^2 \hat{\Delta\xb}\circ\hat{\Delta \sbb}\,,\\
% 	(b)&~~\munew =  [1-\alpha(1-\sig)]\mu - \frac{\alpha\,\vb^\ts\one_\dimtwo}{\dimtwo}.
% %	(c)&~~\rb(\alpha) = (1-\alpha) \rb. 
% 	\end{flalign*}
% 	%
% \end{lemma}
% %
% \begin{proof}
% Proving $(a)$: 
% 	\begin{flalign}
% 	\xnew \circ \snew &= (\xb + \alpha \hat{\Delta\xb}) \circ (\sbb + \alpha \hat{\Delta\sbb})  \notag \\ 
% 	& = \xcircs + \alpha(\xb \circ \hat{\Delta\sbb} + \sbb\circ\hat{\Delta\xb}) + \alpha^2 \hat{\Delta\xb}\circ\hat{\Delta \sbb}  \notag\\
% 	& = \xcircs + \alpha(-\xcircs + \sig\mu \one_\dimtwo - \vb) + \alpha^2\hat{\Delta\xb}\circ\hat{\Delta \sbb}  \notag \\
% 	& = (1-\alpha)\xcircs + \alpha\sig\mu \one_\dimtwo - \alpha\vb + \alpha^2\hat{\Delta\xb}\circ\hat{\Delta \sbb}\,, \notag
% 	\end{flalign} 
% 	%
% 	where the third equality follows from eqn.~\eqref{eq:iip_3_f_3}. Now, left-multiply the above equality by $\one_\dimtwo^\ts$ and divide by $\dimtwo$ to obtain $(b)$. (Notice that $\hat{\Delx}^\ts\hat{\Dels}=0$ from eqns.~\eqref{eq:iip_3_f_1} and \eqref{eq:iip_3_f_2}.)
% \end{proof}

% \noindent Next, we provide an upper bound on $\alpha$, ensuring that each new point $(\xnew,\ynew,\snew)$ traversed by the algorithm stays within the neighborhood $\neigh$.

% \begin{lemma}\label{lemmamaxalpha1_f}
% 	Assume $(\hat{\Delx},\hat{\Dely},\hat{\Dels})$  satisfies eqns. $(\ref{eq:iip_3_f})$ for some $\sig > 0$, $(\xb, \yb,\sbb) \in \neigh$ for $\gamma \in (0,1)$, and $\|\vb\|_2 \leq \frac{\gamma \sig \mu}{4}$. Then, $(\xnew,\ynew,\snew) \in \neigh$ for every scalar $\alpha$ such that 
% 	\begin{flalign} \label{alphalemma1_f}
% 	0 \leq \alpha \leq \min \left\{ 1, \frac{\gamma \sig \mu}{4 \delxdelsnorm}\right\} .
% 	\end{flalign}
% \end{lemma}

% \begin{proof}
% %
% 	First, we show that  $\xnew \circ \snew \geq (1-\gamma) \munew \one_\dimtwo$. From Lemma~\ref{lemmamaxalpha0}, we get
% \begin{flalign}
% &\xnew \circ \snew - (1-\gamma) \munew \one_\dimtwo \notag \\
% &= (1-\alpha)\left(\xcircs - (1-\gamma)\mu\,\one_\dimtwo\right) + \alpha \threefac\, \one_\dimtwo - \alpha \left(\vb - (1-\gamma)\frac{\vb^\ts\one_\dimtwo}{\dimtwo}\one_\dimtwo\right)\nonumber\\
% &~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~+ \alpha^2 \left(\delxdels \right)  \notag \\
% & \geq \alpha \left( \threefac  - \nbr{\vb- (1-\gamma)\frac{\vb^\ts\one_\dimtwo}{\dimtwo}\,\one_\dimtwo}_\infty    - \alpha \nbr{\hat{\Delta\xb}\circ\hat{\Delta\sbb}}_\infty\right) \one_\dimtwo  \notag \\
% & \geq \alpha \Bigg(\threefac - 2 \|\vb\|_\infty -  \alpha\delxdelsnorm \Bigg)\one_\dimtwo \notag \\ 
% & \geq \alpha \Bigg(\threefac - \frac{\threefac}{2} -  \frac{\threefac}{4}\Bigg) \one_\dimtwo  = \, \alpha\frac{\threefac}{4}\one_n\ge\zero \notag.
% \end{flalign} 
% %
% The first inequality follows from $\xcircs\ge(1-\gamma)\mu\,\one_\dimtwo$, because $(\xb,\yb,\sbb)\in\mathcal{N}(\gamma)$ and $\ab\le\|\ab\|_\infty\,\one_\dimtwo$ for any vector $\ab\in\R{\dimtwo}$. The second-to-last inequality follows from the fact that for any $\ub \in \mathbb{R}^\dimtwo$ and $\delta \in [0,\dimtwo]$, $\nbr{\ub - \delta \frac{\ub^\ts \one_\dimtwo}{\dimtwo}\,\one_\dimtwo}_\infty \leq (1+ \delta)\|\ub\|_\infty$. Thus, we prove that the point $(\xnew,\ynew,\snew)$ satisfies the proximity condition for $\neigh$.

% %\agniva{The inequality I used is the following:
% %$\nbr{\vb- (1-\gamma)\frac{\vb^\ts\one_\dimtwo}{\dimtwo}\,\one_\dimtwo}_\infty\le %(2-\gamma)\|\vb\|_\infty\le 2\,\|\vb\|_\infty$. The last inequality holds as $\gamma>0$. %Similarly, $\nbr{\hat{\Delta\xb}\circ\hat{\Delta\sbb} - (1-\gamma) \frac{\delxTdels}{\dimtwo} %\,\one_\dimtwo)}_\infty\le 2\,\|\hat{\Delta\xb}\circ\hat{\Delta\sbb}\|_\infty$. Am I missing %anything?} XXX

% Finally, we show that $(\xnew,\ynew,\snew)\in\mathcal{F}^0$ \ie~it satisfies the primal and dual constraints and $(\xnew,\snew)>\zero$. From eqn.~\eqref{eq:iip_3_f} and the fact that $(\xb,\yb,\sbb)\in\mathcal{F}^0$,  we get $\Ab\,\xnew=\Ab\xb+\alpha\Ab\hat{\Delta\xb}=\bb$. Similarly, $$\Ab^\ts\,\ynew+\snew=(\Ab^\ts\yb+\sbb)+\alpha(\Ab^\ts\hat{\Delta\yb}+\hat{\Delta\sbb})=\Ab^\ts\yb+\sbb = \cbb.$$  
% %
% We now show that $(\xnew,\snew)>\zero$. For $\alpha=0$, we trivially have$(\xnew,\snew)=(\xb,\sbb)>\zero$. To prove $(\xnew,\snew)>\zero$ for $0<\alpha\le1$, we first show $\munew>0$. Using $\gamma \in (0,1)$, the inequality $\abs{\frac{\vb^\ts\one_n}{n}}\le\|\vb\|_\infty\le\|\vb\|_2$, and the assumption $\|\vb\|_2\le\frac{\threefac}{4}$, we get $\frac{\vb^\ts\one_\dimtwo}{\dimtwo} < \frac{\sig \mu}{4}$. 
% Thus, from Lemma~\ref{lemmamaxalpha0}(b), 
% 	\begin{flalign}
% 	\munew &= [1-\alpha(1-\sig)]\mu - \alpha \,\frac{\vb^\ts\one_\dimtwo}{\dimtwo}\nonumber\\
% 	%+ \alpha^2\,\frac{\hat{\Delta\xb}^\ts\hat{\Delta\sbb}}{\dimtwo}\notag \\
% 	&> [1-\alpha(1-\sig)]\mu -  \alpha\,\frac{\sig \mu}{4}\nonumber\\
% 	%+ \alpha^2\,\frac{\hat{\Delta\xb}^\ts\hat{\Delta\sbb}}{\dimtwo} \notag \\
% 	&= (1-\alpha)\mu + \alpha\,\frac{3\,\sig \mu}{4}>0.
% 	\label{last}
% 	\end{flalign} 
% %
% The last inequality holds because $\alpha\in (0,1]$, $\sigma\in (0,1)$, and $\mu>0$. 
% %
% We already have $\xnew\circ\snew\ge (1-\gamma)\munew\one_n$. Combining with $\munew>0$ and $\gamma\in (0,1)$ this implies that $\xnew\circ\snew>\zero$. Therefore, $x_i(\alpha)\,s_i(\alpha)>0$ for all $i=1\dots n$ which implies that, for each $i$, either both $x_i(\alpha)$ and $s_i(\alpha)$ are positive or both $x_i(\alpha)$ and $s_i(\alpha)$ are negative. We will use contradiction to prove that the second case is not possible.

% Indeed, assume that $x_i(\alpha)<0$ and $s_i(\alpha)<0$ for some $i=1 \ldots n$. First, we rewrite $x_i(\alpha)$ and $s_i(\alpha)$ as follows\footnote{Here, $x_i(\alpha)$, $s_i(\alpha)$, $x_i$, $s_i$, $\hat{\Delta x_i}$, and $\hat{\Delta s_i}$ are the $i$-th elements of $\xnew$, $\snew$, $\xb$, $\sbb$, $\hat{\Delx}$, and $\hat{\Dels}$, respectively.}
% %
% \begin{subequations}
% \begin{flalign}
% x_i(\alpha)=&~x_i+\alpha\hat{\Delta x_i}<0\label{eq:x_i},\\
% s_i(\alpha)=&~s_i+\alpha\hat{\Delta s_i}<0\label{eq:s_i}.
% \end{flalign}
% \end{subequations}
% %
% Recall that both $x_i$ and $s_i$ are positive. Therefore, pre-multiplying eqn.~\eqref{eq:x_i} by $s_i$ and eqn.~\eqref{eq:s_i} by $x_i$ we get
% %
% \begin{subequations}
% \begin{flalign}
% x_is_i+\alpha s_i\hat{\Delta x_i}<&~0\label{eq:x_i1},\\
% x_is_i+\alpha x_i\hat{\Delta s_i}<&~0\label{eq:s_i1}.
% \end{flalign}
% \end{subequations}
% %
% Adding eqns.~\eqref{eq:x_i1} and \eqref{eq:s_i1} and applying eqn.~\eqref{eq:iip_3_f_3} (element-wise), we get
% %
% \begin{flalign}
% &~2x_is_i+\alpha (s_i\hat{\Delta x_i}+x_i\hat{\Delta s_i})<0\nonumber\\
% \Rightarrow&~2x_is_i+ \alpha (-x_is_i+\sigma\mu-v_i)<0\nonumber\\
% \Rightarrow&~ (2-\alpha)x_is_i+\alpha\sigma\mu-\alpha v_i<0\nonumber\\
% \Rightarrow&~ v_i>\frac{2-\alpha}{\alpha}x_is_i+\sigma\mu > \sigma\mu\label{eq:xs}.
% \end{flalign}
% %
% In the above $v_i$ is the $i$-th element of $\vb$; the first inequality in eqn.~\eqref{eq:xs} holds because $\alpha>0$; the second inequality in eqn.~\eqref{eq:xs} because $\frac{2-\alpha}{\alpha}x_is_i>0$ ($x_i,s_i>0$ and $0 < \alpha \leq 1$). Using $\|\vb\|_2\le\frac{\threefac}{4}$ we get
% %
% $$v_i\le\|\vb\|_\infty\le\|\vb\|_2\le\frac{\threefac}{4}<\sigma\mu\,,$$
% %
% for all $i=1\ldots n$. This contradicts the inequality of eqn.~\eqref{eq:xs}; thus, both $x_i(\alpha)>0$ and $s_i(\alpha)>0$ for all $i=1\ldots n$ and all $\alpha\in[0,1]$.
% %
% \end{proof}

% \noindent We now turn to the task of providing a lower bound on the values of $\alphaused$ and the corresponding $\mu(\alphaused)$ value. 
% %
% \begin{lemma}[Lemma 3.6 of \cite{Mon03}]\label{lemmaminalpha1_f}
% 	At each iteration of the feasible IPM algorithm, if $\|\vb\|_2\le\frac{\gamma\sigma\mu}{4}$, then the step size $\alphaused$ satisfies 
% 	\begin{flalign} \label{alphalemma2_f}
% 	\alphaused \geq \min \left\{ 1,  \frac{ \min   \{ \gamma \sigma, (1 - \frac{5}{4} \sigma) \} \mu } {4  \|\hat{\Delta x} \circ \hat{\Delta s}\|_\infty}  \right\} 
% 	\end{flalign}
% 	and 
% 	\begin{flalign} \label{mulemma2_f}
% 	\mu(\alphaused)= \Big[ 1 - \frac{\alphaused}{2} (1-\frac{5}{4}\sig) \Big] \mu. 
% 	\end{flalign}
% \end{lemma}
% %
% \noindent At this point, we have provided a lower bound (eqn.~(\ref{alphalemma2_f})) for the allowed values of the step size $\alphaused$. Next, we will show that this lower bound is bounded away from zero. From eqn.~(\ref{alphalemma2_f}), is suffices to show that $\delxdelsnorm$ is bounded. First, we state the following inequality that will be instrumental in proving Lemma~\ref{lemmaminalpha2_f}.

% \begin{lemma}\label{prop:wri}
% 	Let $\ab,\bb\in\R{n}$ be any two vectors such that $\ab^\ts\bb\ge 0$. Then
% 	\begin{flalign*}
% 	\|\ab\circ\bb\|_2\le \|\ab+\bb\|_2^2\,.
% 	\end{flalign*}
% \end{lemma}
% %
% \noindent See~\cite{wright1997primal} for a proof of Lemma~\ref{prop:wri}; as a matter of fact,~\cite{wright1997primal} proved $\|\ab\circ\bb\|_2\le2^{-3/2}\|\ab+\bb\|_2^2$, which is tighter. This tighter bound is not needed in our proof. 

% \begin{lemma}\label{lemmaminalpha2_f}
% 	Let $(\xb,\yb,\sbb) \in \neigh$ and $\|\vb\|_2\le\frac{\gamma\sigma\mu}{4}$. Then   $(\hat{\Delta \xb},\hat{\Delta \yb},\hat{\Delta \sbb})$ satisfies 
	
% \begin{flalign} \label{normsmax_f}
% \|\hat{\Delx}\circ\hat{\Dels}\|_\infty\le\left(1+\frac{\sigma^2}{1-\gamma}\right)n\mu + \frac{\gamma^2\sigma^2}{16(1-\gamma)}\mu+\frac{\gamma\sigma^2}{2}\mu\,.
% \end{flalign}
% \end{lemma}

% \begin{proof}
% First, we multiply eqn.~(\ref{eq:iip_3_f_3}) on the left by $(\Xb \Sb)^{-1/2}$ to get
% %
% \begin{flalign}\label{eq:Dint}
% \Db^{-1} \hat{\Delta \xb} + \Db \hat{\Delta \sbb} = -(\Xb \Sb)^{1/2}\one_\dimtwo + 
% \sig \mu (\Xb \Sb)^{-1/2} \one_\dimtwo - (\Xb \Sb)^{-1/2} \vb\,.
% \end{flalign} 
% %
% Next, pre-multiplying eqn.~\eqref{eq:iip_3_f_2} by $\hat{ \Delta \xb}^\ts$ and applying eqn.~\eqref{eq:iip_3_f_1}, we have $\hat{\Delx}^\ts\hat{ \Delta \sbb}=0$. This also implies that $\hat{\Delx}^\ts\hat{ \Delta \sbb}=(\Db^{-1}\hat{\Delx})^\ts(\Db\hat{ \Delta \sbb})$. Applying Lemma~\ref{prop:wri} with $\ab=\Db^{-1}\hat{\Delx}$ and $\bb=\Db\hat{\Dels}$, and using eqn.~\eqref{eq:Dint} we get
% %
% \begin{flalign}
% \|\hat{ \Delta \xb}\circ\hat{ \Delta \sbb}\|_2=&~\|(\Db^{-1}\hat{ \Delta \xb})\circ(\Db\hat{ \Delta \sbb})\|_2\le\|\Db^{-1} \hat{\Delta \xb} + \Db \hat{\Delta \sbb}\|_2^2\nonumber\\
% =&~\|-(\Xb \Sb)^{1/2}\one_\dimtwo + 
% \sig \mu (\Xb \Sb)^{-1/2} \one_\dimtwo - (\Xb \Sb)^{-1/2} \vb\|_2^2\nonumber\\
% =&~\|(\Xb \Sb)^{1/2}\one_\dimtwo+(\Xb \Sb)^{-1/2}(\vb-\sigma\mu\one_\dimtwo)\|_2^2\nonumber\\
% =&~\|(\Xb \Sb)^{1/2}\one_\dimtwo\|_2^2+ 2\cdot\one_\dimtwo^\ts(\vb-\sigma\mu\one_\dimtwo)+\|(\Xb \Sb)^{-1/2}(\vb-\sigma\mu\one_\dimtwo)\|_2^2\nonumber\\
% \le&~n\mu+2n (\|\vb\|_2-\sigma\mu)+\|(\Xb \Sb)^{-1/2}(\vb-\sigma\mu\one_\dimtwo)\|_2^2\label{eq:dineq}.
% \end{flalign}
% %
% The inequality in eqn.~\eqref{eq:dineq} follows from $\|(\Xb \Sb)^{1/2}\one_\dimtwo\|_2^2=n\mu$ and $\abs{\one_\dimtwo^\ts\vb}\le n\,\|\vb\|_\infty\le n\,\|\vb\|_2$. Next, consider the last term on the right hand side of eqn.~\eqref{eq:dineq}:
% %
% \begin{flalign}
% \|(\Xb \Sb)^{-1/2}(\vb-\sigma\mu\one_\dimtwo)\|_2^2=&~\|(\Xb \Sb)^{-1/2}\vb\|_2^2+\sigma^2\mu^2\|(\Xb \Sb)^{-1/2}\one_\dimtwo\|_2^2-2\sigma\mu\,\one_n^\ts(\Xb\Sb)^{-1}\vb\nonumber\\
% \le&~\frac{\|\vb\|_2^2}{\min_i x_is_i}+\sigma^2\mu^2\sum_{i=1}^{n}\frac{1}{x_is_i}-2\sigma\mu\sum_{i=1}^{n}\frac{v_i}{x_is_i}.\label{eq:dint2}
% \end{flalign}
% %
% Eqn.~\eqref{eq:dint2} follows from $\|(\Xb \Sb)^{-1/2}\vb\|_2^2\le\|(\Xb \Sb)^{-1/2}\|_2^2\|\vb\|_2^2$ and $\|(\Xb \Sb)^{-1/2}\|_2^2=\nicefrac{1}{\min_i x_is_i}$. Moreover, it is easy to verify that $\|(\Xb \Sb)^{-1/2}\one_\dimtwo\|_2^2=\sum_{i=1}^{n}\nicefrac{1}{x_is_i}$ and $\one_n^\ts(\Xb\Sb)^{-1}\vb=\sum_{i=1}^{n}\nicefrac{v_i}{x_is_i}$. Now, we have $x_is_i\ge(1-\gamma)\mu$ for $i=1 \ldots n$ as $(\xb,\yb,\sbb)\in\mathcal{N}(\gamma)$. Also, $x_is_i\le\sum_{i=1}^{n}x_is_i=n\mu$. Using the above we rewrite eqn.~\eqref{eq:dint2} as 
% %
% \begin{flalign}
% \|(\Xb \Sb)^{-1/2}(\vb-\sigma\mu\one_\dimtwo)\|_2^2\le\frac{\|\vb\|_2^2}{(1-\gamma)\mu}+\frac{n\sigma^2\mu^2}{(1-\gamma)\mu}-2\sigma\mu\frac{\sum_{i=1}^{n}v_i}{n\mu}.\label{eq:dint3}
% \end{flalign}
% %
% Combining eqns.~\eqref{eq:dineq} and~\eqref{eq:dint3} we get
% %
% \begin{flalign}
% \|\hat{ \Delta \xb}\circ\hat{ \Delta \sbb}\|_2\le&~ n\mu+2n (\|\vb\|_2-\sigma\mu)+\frac{\|\vb\|_2^2}{(1-\gamma)\mu}+\frac{n\sigma^2\mu}{(1-\gamma)}-2\sigma\frac{\sum_{i=1}^{n}v_i}{n}\nonumber\\
% =&~\left(1+\frac{\sigma^2}{1-\gamma}\right)n\mu+2n (\|\vb\|_2-\sigma\mu)+\frac{\|\vb\|_2^2}{(1-\gamma)\mu}-2\sigma\frac{\sum_{i=1}^{n}v_i}{n}\,.\label{eq:dint4}
% \end{flalign}
% %
% Using  $\|\vb\|_2\le\frac{\gamma\sigma\mu}{4}$ and the fact that $\abs{\nicefrac{\vb^\ts\one_n}{n}}\le\|\vb\|_\infty\le\|\vb\|_2$, we get
% \begin{flalign}
% \|\hat{ \Delta \xb}\circ\hat{ \Delta \sbb}\|_2\le\left(1+\frac{\sigma^2}{1-\gamma}\right)n\mu+\frac{\gamma^2\sigma^2}{16 (1-\gamma)}\mu+\frac{\gamma\sigma^2}{2}\mu.
% \end{flalign}
% %
% Finally, we conclude the proof using $\|\hat{ \Delta \xb}\circ\hat{ \Delta \sbb}\|_\infty\le\|\hat{ \Delta \xb}\circ\hat{ \Delta \sbb}\|_2$.
% \end{proof}

% \begin{theorem}\label{theoremOuter_f}
% Assume that the constants $\gamma$ and $\sigma$ are such that $\max\{\gamma^{-1},(1-\gamma)^{-1},\sigma^{-1},(1-\frac{5}{4}\sigma)^{-1}\}=\Ocal(1)$. At each iteration of the feasible IPM algorithm, if $\|\vb\|_2\le\frac{\gamma\sigma\mu}{4}$, then after 
% 	$k=\mathcal{O}(\dimtwo \log{\nicefrac{1}{\epsilon}})$ iterations, $(\xb^{k}, \sbb^{k}, \yb^{k})$ satisfies $$\mu_k \leq \epsilon \mu_0.$$
% \end{theorem}

% \begin{proof}
% From Lemma~\ref{lemmaminalpha2_f}, 
% %
% \begin{flalign}
% &~\|\hat{\Delx}\circ\hat{\Dels}\|_\infty\le \left(1+\frac{\sigma^2}{1-\gamma} + \frac{\gamma^2\sigma^2}{16(1-\gamma)}+\frac{\gamma\sigma^2}{2}\right)n\mu\nonumber\\
% \Rightarrow&~\mu\|\hat{\Delx}\circ\hat{\Dels}\|_\infty^{-1}\ge n^{-1} \left(1+\frac{\sigma^2}{1-\gamma} + \frac{\gamma^2\sigma^2}{16(1-\gamma)}+\frac{\gamma\sigma^2}{2}\right)^{-1}.\label{eq:step1}
% \end{flalign}
% %
% Combining eqns.~\eqref{alphalemma2_f} and \eqref{eq:step1} we get
% %
% \begin{flalign}
% 	\alphaused \geq \min \left\{ 1,  \frac{ \min   \{ \gamma \sigma, (1 - \frac{5}{4} \sigma) \} } {4  \,n \left(1+\frac{\sigma^2}{1-\gamma} + \frac{\gamma^2\sigma^2}{16(1-\gamma)}+\frac{\gamma\sigma^2}{2}\right)}  \right\}.\label{eq:step2}
% \end{flalign}
% %
% Let $\max\{\gamma^{-1},(1-\gamma)^{-1},\sigma^{-1},(1-\frac{5}{4}\sigma)^{-1}\}\le \lambda$ for some constant $\lambda> 1$. Therefore, $\gamma\sigma\ge\frac{1}{\lambda^2}$ and $(1-\frac{5}{4}\sigma)\ge\frac{1}{\lambda}$, which further implies that $\min\{ \gamma \sigma, (1 - \frac{5}{4} \sigma)\}\ge\min\{\frac{1}{\lambda},\frac{1}{\lambda^2}\}=\frac{1}{\lambda^2}$. Also, $\frac{1}{1-\gamma}\le\lambda$. Combining these with eqn.~\eqref{eq:step2}, we get
% %
% \begin{flalign}
% \alphaused\ge\min\left\{1,\frac{\frac{1}{\lambda^2}}{4n (1+\lambda\sigma^2+\frac{\lambda\gamma^2\sigma^2}{16}+\frac{\gamma\sigma^2}{2})}\right\}=\min\left\{1,\frac{1}{4n(\lambda^2+\lambda^3\sigma^2+\frac{\lambda^3\gamma^2\sigma^2}{16}+\frac{\lambda^2\gamma\sigma^2}{2})}\right\}.\label{eq:step3}
% \end{flalign}
% %
% Note that in eqn.\eqref{eq:step3}, $4n(\lambda^2+\lambda^3\sigma^2+\frac{\lambda^3\gamma^2\sigma^2}{16}+\frac{\lambda^2\gamma\sigma^2}{2})>$. Thus,
% \begin{flalign}
% &~\alphaused\ge \frac{1}{4n(\lambda^2+\lambda^3\sigma^2+\frac{\lambda^3\gamma^2\sigma^2}{16}+\frac{\lambda^2\gamma\sigma^2}{2})}\nonumber\\
% \Rightarrow&~ \frac{\alphaused}{2}\left(1-\frac{5}{4}\sigma\right)\ge \frac{1-\frac{5}{4}\sigma}{8n(\lambda^2+\lambda^3\sigma^2+\frac{\lambda^3\gamma^2\sigma^2}{16}+\frac{\lambda^2\gamma\sigma^2}{2})}\ge \frac{1}{8n\lambda^3(1+\lambda\sigma^2+\frac{\lambda\gamma^2\sigma^2}{16}+\frac{\gamma\sigma^2}{2})}=\frac{\beta}{n}\,,\label{eq:step4}
% \end{flalign}
% %
% where 
% %
% \begin{equation}\label{eqn:pdbeta1}
% \beta=\frac{1}{8\lambda^3(1+\lambda\sigma^2+\frac{\lambda\gamma^2\sigma^2}{16}+\frac{\gamma\sigma^2}{2})}.
% \end{equation}
% %
% We also note that the second inequality in eqn.~\eqref{eq:step4} holds because $1-\frac{5}{4}\sigma\ge\frac{1}{\lambda}$. Let $\mu=\mu_k$ and $\mu(\alphaused)=\mu_{k+1}$ in eqn.~\eqref{mulemma2_f};  applying eqn.~\eqref{eq:step4}, we get
% %
% \begin{flalign} \label{lem:conv}
% \mu_{k+1} \leq  \left(1 - \frac{\beta}{\dimtwo}\right) \mu_k, \forall k \geq 0.
% \end{flalign}
% %
% Applying the above inequality recursively,  we get $\mu_{k} \leq  \left(1 - \frac{\beta}{\dimtwo}\right)^k \mu_0$. Therefore, for any accuracy parameter $\epsilon\in(0,1)$, $\mu_{k}\le\epsilon\mu_0$ holds, if $\left(1 - \frac{\beta}{\dimtwo}\right)^k\le \epsilon$ holds. Thus, it suffices for $k$ to be at least
% %
% \begin{flalign}
% k\ge \frac{n}{\beta}\log (\nicefrac{1}{\epsilon}).
% \end{flalign}
% %
% Therefore, since $\beta$, as defined in eqn.~(\ref{eqn:pdbeta1}), is a constant,  we need $\Ocal(n\log\frac{1}{\epsilon})$ iterations to satisfy $\mu_k\le \epsilon\mu_0$.
% \end{proof}

==> X_infeasible.tex <==
% In order to avoid spurious solutions, primal-dual path-following IPMs bias the search direction towards the \emph{central path} and restrict the iterates to a neighborhood of the central path. This search is controlled by the \emph{centering parameter} $\sigma\in[0,1]$.
% %  Setting $\sigma$ close to one results in short-step IPMs, which have the best theoretical behavior but poor practical performance; setting $\sigma$ far from one results in long-step IPMs, which have somewhat worse theoretical behavior,  but  work  well  in  practice;  alternating  between steps with $\sigma$ close and far from one results in predictor-corrector algorithms that are a compromise between the two approaches; see () for details.
% %
% At each iteration, given the current solution $(\xb^{k},\yb^{k},\sbb^{k})$, a standard infeasible IPM obtains the search direction $(\Delta\xb^k,\Delta\yb^k,\Delta\sbb^k)$ by solving the following system of linear equations:
% \begin{subequations}\label{eq:system}
% 	\begin{flalign}
% 		\Ab\Db^2\Ab^\ts\Delta\yb^k=~&\pb^k\,,\label{eq:normal1}\\
% 		\Delta\sbb^k=~&-\rb^k_d-\Ab^\ts\Delta\yb^k\,,\label{eq:dels}\\
% 		\Delta\xb^k=~&-\xb^k+\sigma\mu_k\Sb^{-1}\one_\dimtwo-\Db^2\Delta\sbb^k.\label{eq:delx}
% 	\end{flalign}
% \end{subequations}
% %
% Here $\Db$ and $\Sb$ are computed given the current iterate $(\xb^{k}$ and $\sbb^{k})$; we skip the indices on $\Db$ and $\Sb$ for notational simplicity. 
% %\haim{Perhaps give $\Db$ and $\Sb$ an index?} 
% After solving the above system, the infeasible IPM Algorithm~\ref{algo:iipm} proceeds by computing a step-size $\alphabar$ to return:
% %
% \begin{flalign}\label{eqn:update}
% 	%
% 	(\xb^{k+1},\yb^{k+1},\sbb^{k+1}) = (\xb^{k},\yb^{k},\sbb^{k}) + \alphabar (\Delta \xb^k,\Delta \yb^k,\Delta \sbb^k).
% 	%
% \end{flalign}
% %
% Recall that $\rb^k=(\rb^k_p,\rb^k_d)$ is a vector with  $\rb^k_p=\Ab\xb^k-\bb$ and $\rb^k_d=\Ab^\ts\yb^k+\sbb^k-\cbb$ (the primal and dual residuals). We also use the \textit{duality measure} $\mu_k=\nicefrac{{\xb^k}^\ts\sbb^k}{n}$ and the vector
% %
% \begin{flalign}\label{eqn:pdef}
% 	%
% 	\pb^k&=-\rb_p^k-\sigma\mu_k\Ab\Sb^{-1}\one_\dimtwo+\Ab\xb^k-\Ab\Db^2\rb^k_d.
% 	%
% \end{flalign}
% %
% Given $\Delta\yb^k$ from eqn.~(\ref{eq:normal1}), $\Delta\sbb^k$ and $\Delta\xb^k$ are easy to compute from eqns.~\eqref{eq:dels} and \eqref{eq:delx}, as they only involve matrix-vector products.  However, since we  use Algorithm~\ref{algo:PCG} to solve eqn.~\eqref{eq:normal1} approximately using the sketching-based preconditioned CG solver, the primal and dual residuals \textit{do not} lie on the line segment between $\zero$ and $\rb^0$. This invalidates known proofs of convergence for infeasible IPMs.

% For notational simplicity, we now drop the dependency of vectors and scalars on the iteration counter $k$. Let $\hat{\Delta \yb}=\Qb^{\nicefrac{-1}{2}}\tilde{\zb}^t$ be the approximate solution to eqn.~(\ref{eq:normal1}). In order to account for the loss of accuracy due to the approximate solver, we compute $\hat{\Delta\xb}$ as follows:
% %
% \begin{flalign}
% 	\hat{\Delta\xb}=~-\xb+\sigma\mu\Sb^{-1}\one_\dimtwo-\Db^2\hat{\Delta\sbb}-\Sb^{-1}\vb\label{eq:delxhat}.
% \end{flalign}
% %
% Here $\vb\in\R{n}$ is a perturbation vector that needs to exactly satisfy the following invariant at each iteration of the infeasible IPM:
% %
% \begin{flalign}
% 	%
% 	\Ab\Sb^{-1}\vb=\Ab\Db^2\Ab^\ts\hat{\Delta\yb}-\pb\,\label{eq:addl}.
% 	%
% \end{flalign}
% %
% We note that the computation of $\hat{ \Delta \sbb}$ is still done using, essentially, eqn.~\eqref{eq:dels}, namely
% %
% \begin{flalign}
% %
% \Delta\hat{\sbb}^k=~&-\rb^k_d-\Ab^\ts\hat{\Delta\yb}^k.\label{eq:delshat}
% %
% \end{flalign}
% %
% In \citep{Mon03} it is argued that if $\vb$ satisfies eqn.~\eqref{eq:addl}, the primal and dual residuals lie in the correct line segment.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% We are now ready to present the infeasible IPM algorithm. We will need the following definition for the neighborhood
% {\small\begin{flalign}
% 		&\mathcal{N}(\gamma)=\Big\{(\xb^k,\yb^k,\sbb^k):x_i^k s_i^k\ge(1-\gamma)\mu\,~\text{and}~\,\frac{\|\rb^k\|_2}{\|\rb^0\|_2} \leq \frac{\mu_k}{\mu_0},\Big\}.\nonumber
% \end{flalign}}
% %
% Here $\gamma \in (0,1)$ and we note that the duality measure $\mu_k$ steadily reduces at each iteration.

% \begin{algorithm}[H]
% 	\caption{Infeasible IPM}\label{algo:iipm}%
% 	\begin{algorithmic}
		
% 		\State \textbf{Input:}
% 		$\Ab\in\RR{\dimone}{\dimtwo}$,  $\bb\in\R{\dimone}$, $\cbb\in\R{\dimtwo}$, $\gamma \in (0,1)$, tolerance $\epsilon> 0$, centering parameter $\sig\in (0,\nicefrac{4}{5})$;
		
% 		\vspace{1mm}
% 		\State \textbf{Initialize:} $k\gets 0$; initial point $(\xb^{0},\yb^{0},\sbb^{0})$;
		
% 		%------------------------------------------------------
% 		\vspace{1mm}
% 		\While{$\mu_k > \epsilon$}
% 		%\begin{enumerate}
% 		%[(a)]
% 		%\State (a) $(\xb,\yb,\sbb):=(\xb^{k},\yb^{k},\sbb^{k});$ %$\rb=(\rb_p,\rb_d)=(\Ab\xb-\bb,\Ab^\ts\yb+\sbb-\cbb)$ and
% 		%and choose $\sig \in (0,\nicefrac{4}{5})$.
% 		%\item Let $\Db= \Xb^{\nicefrac{1}{2}}\Sb^{-\nicefrac{1}{2}} \eb$ and $\rb=(\rb_p,\rb_d)=(\Ab\xb-\bb,\Ab^\ts\yb+\sbb-\cbb)$.
% 		%                 \begin{flalign}
% 		%                 \rb_p &= -\Ab \xb - b \\
% 		%                 \rb_d & = \Ab^T \yb+\sbb - c \\
% 		%                 \rb & =  (\rb_p,\rb_d)
% 		%                 \end{flalign}
		
% 		\vspace{1mm}
% 		\State (a)~Compute sketching matrix $\Wb \in \mathbb{R}^{n \times w}$ (Section~\ref{sxn:background}) with $\zeta=1/2$ and $\delta = O(n^{-2})$;
% 		\vspace{1mm}
% 		\State (b)~Compute $\rb_p^k=\Ab\xb^k-\bb$; $\rb_d^k=\Ab^\ts\yb^k+\sbb^k-\cbb$; and $\pb^k$ from eqn.~(\ref{eqn:pdef});
% 		\vspace{1mm}
% 		\State (c)~Solve the linear system of eqn.~\eqref{eq:precond_alt} for $\zb$ using Algorithm~\ref{algo:PCG} with $\Wb$ from step (a) and $t=\Ocal(\log n)$. Compute $\hat{\Delta \yb}=\Qb^{\nicefrac{-1}{2}}{\zb}$;
% 		\vspace{1mm}
% 		\State (d)~Compute $\vb$ using eqn.~\eqref{eq:compv} with $\Wb$ from step (a); $\hat{\Delta\sbb}$ using eqn.~\eqref{eq:dels}; $\hat{\Delta\xb}$ using eqn.~\eqref{eq:delxhat};
% 		\vspace{1mm}
% 		\State (e)~\label{stepalpha1} Compute $\alphamax = \argmax\{ \alpha \in [0,1] : (\xb^k,\yb^k,\sbb^k) + \alpha (\hat{\Delta \xb}^k,\hat{\Delta \yb}^k,\hat{\Delta \sbb}^k)  \in \neigh\}$.
% 		\vspace{1mm}
% 		\State (f)~\label{stepalpha2}Compute $\alphaused = \argmin\{\alpha \in [0, \alphamax]: (\xb^k + \alpha \hat{\Delta \xb}^k)^\ts (\sbb^k + \alpha \hat{\Delta\sbb}^k)\}$.
% 		\vspace{1mm}
% 		\State (g)~Compute $(\xb^{k+1}, \yb^{k+1}, \sbb^{k+1}) = (\xb^k,\yb^k,\sbb^k) + \alphabar (\hat{\Delta \xb}^k,\hat{\Delta \yb}^k,\hat{\Delta \sbb}^k)$; set $k \gets k + 1$;
		
% 		\EndWhile
% 	\end{algorithmic}
% \end{algorithm}
